Challenges in Context-Aware Neural Machine Translation

Context-aware neural machine translation involves leveraging information beyond sentence-level context to resolve inter-sentential discourse dependencies and improve document-level translation quality, and has given rise to a number of recent techniques. However, despite well-reasoned intuitions, most context-aware translation models show only modest improvements over sentence-level systems. In this work, we investigate several challenges that impede progress within this field, relating to discourse phenomena, context usage, model architectures, and document-level evaluation. To address these problems, we propose a more realistic setting for document-level translation, called paragraph-to-paragraph (para2para) translation, and collect a new dataset of Chinese-English novels to promote future research.

==> tables/attention_visual.tex <==
\begin{table}[t]
\centering
\resizebox{1.0\columnwidth}{!}
{%
\begin{tabular}{l}\toprule
\begin{tabular}[c]{@{}l@{}}Context: \begin{CJK*}{UTF8}{gbsn}他的嗓音低沉，其中的含义让人心中一凛。\end{CJK*}\\ Source : 
\hlc[cyan!50]{$\llbracket ? \rrbracket$ }\begin{CJK*}{UTF8}{gbsn}那语气带着某种嘲讽...\end{CJK*}\\ Target  : \hlc[pink]{His} tone seemed to contain some sort of ridicule...\end{tabular} \\\hline
\end{tabular}}
\caption{An example of pronoun ellipsis, where the \hlc[pink]{highlighted} pronoun needs context to disambiguate the gender of the pronoun in the target sentence, \hlc[cyan!50]{$\llbracket ? \rrbracket$ } is an omitted pronoun. }
\label{tab:pronoun-case}
\vspace{-1mm}
\end{table} 


==> tables/automatic_metric.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{llllllllll}
\toprule
&&    & BLEU & \multicolumn{5}{c}{BLONDE}   & COMET \\ \midrule
&&    & & all & pronoun & entity & tense & dm & \\ \midrule
\multicolumn{1}{c}{\text{ZH}\rightarrow \text{EN}}
&\multicolumn{1}{c}{XFMR}  
& baseline & 19.97 & 36.84 & 69.62 & 50.34 & 71.17 & 57.28 & 0.2302\\
& 1-2  & x     & x     & x     & x     & x     & x     & x \\
& 2-2  & 19.66 & 35.45 & 73.74 & 48.23 & 70.01 & 55.77 & 0.2208 \\
& 2-2-shuffle  & 20.01 & 36.94 & 73.62 & 50.17 & 71.28 & 57.53  & 0.2517 \\
& 3-1         & 19.59 & 35.99 & 75.01 & 45.08 & 70.98          & 57.04       & 0.2237 \\
& 3-1-shuffle & 20.30 & 36.59 & 71.47 & 47.80 & 71.28          & 58.16       & 0.2245 \\ 
&\multicolumn{1}{c}{MEGA}
& baseline         & 19.74 & 35.82 & 71.81 & 43.77 & 72.05          & 57.72       & 0.2467 \\
\multicolumn{1}{c}{}                               
& 1-2          & 19.59 & 34.49 & 71.30 & 35.26 & 71.79          & 57.57       & 0.2446 \\
\multicolumn{1}{c}{}                               
& 2-2          & 19.07 & 36.24 & 68.99 & 51.49  & 70.91          & 54.16       & 0.1967 \\
\multicolumn{1}{c}{}                               
& 3-1        & 19.15 & 34.56 & 72.99 & 34.48   & 70.12          & 57.38       & 0.2120  \\ \bottomrule
\end{tabular}
\caption{Automatic metric results for the sentence-level baseline and concatenation-based settings using the Transformer (XFMR) and MEGA~\citep{ma2023mega} models. \todo{report avg, sd of multiple runs}}
\label{tab:automatic_results}
\end{table*}

==> tables/dm_examples.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{ll}\toprule
\textbf{Type}  & \textbf{Examples} \\
contrast       & but, while, however, although, though, yet, whereas, in contrast, by comparison, conversely  \\
cause          & so, thus, hence, as a result, therefore, thereby, accordingly, consequently, for this reason \\
condition      & if, as long as, provided that, assuming that, given that                                     \\
conjunction    & also, in addition, moreover, additionally, besides, else, plus, furthermore                  \\
(a)synchronous & when, after, then, before, until, after, once, after, next    \\\bottomrule                 
\end{tabular}
\caption{Examples of different discourse marker types.}
\label{tab:dm_example}
\end{table}

==> tables/dp_examples.tex <==
\begin{table*}[t!]
\centering
\begin{tabular}{ll}\toprule
\begin{tabular}[c]{@{}l@{}}Ctx: \begin{CJK*}{UTF8}{gbsn} 他的嗓音低沉，其中的含义让人心中一凛。\end{CJK*}\\ Src: \hlc[cyan!50]{\{?\}} \begin{CJK*}{UTF8}{gbsn} 那语气带着某种嘲讽...\end{CJK*}\\ Tgt: \hlc[pink]{His} tone seemed to contain some sort of ridicule...\end{tabular}           
& Pronoun Ellipsis  \\\hline

% \begin{tabular}[c]{@{}l@{}}  пальчиков не оказалось в АДИС  не ловили . \end{tabular}  & Pronoun Formality \\\hline
\begin{tabular}[c]{@{}l@{}}Ctx: \begin{CJK*}{UTF8}{gbsn} 乔恋还在思考沈良川说过的话。\end{CJK*}\\ Src: \begin{CJK*}{UTF8}{gbsn} 但是她不明白沈良川这么说是为了什么。\end{CJK*}\\ Tgt: But she doesn't understand why did \hlc[pink]{Shen Laingchuan} say that.\end{tabular} 
& Lexical Cohesion  \\\hline

\begin{tabular}[c]{@{}l@{}}Ctx: \begin{CJK*}{UTF8}{gbsn} 因为天气预报说今天有可能会下雨。\end{CJK*}\\ Src: \begin{CJK*}{UTF8}{gbsn} 所以我出门带了雨伞。\end{CJK*}\\ Tgt: \hlc[cyan!50]{\{So\}} I brought umbrella today. \end{tabular} 
& Discourse Marker  \\\hline

\begin{tabular}[c]{@{}l@{}}Ctx:\\ Src:\\ Tgt:\end{tabular}  
& Tense \\\bottomrule           
\end{tabular}
\caption{Examples of discourse phenomena that need context to be accurately translated. \hlc[cyan!50]{Highlighted} are omitted words, \hlc[pink]{Highlighted} are words that need context for either accuracy or consistency. }
\label{tab:dp}
\end{table*} 

==> tables/ner_accuracy.tex <==
\begin{table}[h]
\centering
\begin{tabular}{llll}\\\toprule
         & baseline & 3-1*  & 3-1*+ \\\hline
Acc. (\%) & 63.61    & 52.54 & 57.90 \\\bottomrule     
\end{tabular}
\caption{Name entity accuracy$(\%)$ analysis on BWB, 3-1*+ is the 3-1* model with shuffled dataset.}
\label{tab:ne_accuracy}
\end{table}

==> tables/shuffled_res.tex <==
\begin{table}[h]
\centering
\resizebox{1.0\columnwidth}{!}
{%
\begin{tabular}{lllllllll}
\toprule
&    & BLEU & \multicolumn{5}{c}{BlonDe}   & COMET \\ \midrule
&    & & all & pron. & entity & tense & d.m. & \\ \midrule
\multicolumn{1}{c}{\multirow{4}{*}{Zh}}
& 1-1 & \bf{20.75} & \bf{36.76} & 73.64 & \bf{44.21} & 72.98 & 60.06 & 0.2454 \\ 
& 2-2 & 20.30 & 35.94  & \bf{77.41} & 37.33  & \bf{73.47} & \bf{60.36} & \bf{0.2471} \\
& 2-2-\it{sf}  & 19.77 & 34.64  & 72.76 & 32.79  & 72.90 & 59.69 & 0.2251 \\
& 3-1 & 19.24 & 35.49  & 76.43 & \bf{39.92}  & 73.01 & 58.80 & 0.2172 \\
& 3-1-\it{sf} & 19.12 & 35.45  & 73.20 & 43.20  & 72.32 & 59.00 & 0.1776 \\
\midrule
\multicolumn{1}{c}{\multirow{4}{*}{Fr}} 
& 1-1 &  35.67 & 47.45 & 74.68 & 63.87 & 76.08 & \bf{79.62} & 0.5000 \\
& 2-2  & \bf{36.21} & \bf{48.66} & \bf{80.69} & \bf{69.46} & \bf{76.65} & 77.92 & 0.5056 \\
& 2-2-\it{sf} & 35.68 & 46.59 & 69.46 & 62.39 & 75.76 & 77.75 & 0.4540 \\
& 3-1 & 35.63	&	47.31	&	76.84	&	62.03	&	75.85	&	78.77	&	\bf{0.5087} \\
& 3-1-\it{sf} & 34.40 & 46.08 & 71.81 & 61.80 & 75.14 & 78.87 & 0.4297 \\
\midrule
\multicolumn{1}{c}{\multirow{4}{*}{De}} 
& 1-1 & \bf{31.12} & \bf{48.23} & 73.36 & \bf{62.72} & 71.84 & \bf{75.95} & 0.3675 \\
& 2-2 & 29.87 & 46.94 & \bf{80.00} & 59.38 & 71.65 & 75.30 & 0.3202 \\
& 2-2-\it{sf} & 28.64 & 44.41 & 72.47 & 52.63 & 70.49 & 72.15 & 0.2498 \\
& 3-1 & 31.11	&	48.13	&	76.10	&	61.45	&	\bf{72.63}	&	75.27	&	\bf{0.3729} \\
& 3-1-\it{sf} & 30.56 & 47.30 & 73.30 & 60.51 & 71.77 & 74.52 & 0.3221\\
\bottomrule
\end{tabular}}
\caption{Automatic metric results across different context-aware translation settings from \{Zh, Fr, De\}$\rightarrow$En.
\textit{sf} means that the model is provided with randomly sampled sentences as context during inference.  
}
\label{tab:sf-res}
\vspace{-3mm}
\end{table}
